Learning to Collaborate by Grouping: a Consensus-oriented Strategy for Multi-agent Reinforcement Learning

Multi-agent systems require effective coordination between groups and individuals to achieve common goals. However, current multi-agent reinforcement learning (MARL) methods primarily focus on improving individual policies and do not adequately address group-level policies, which leads to weak cooperation. To address this issue, we propose a novel Consensus-oriented Strategy (CoS) that emphasizes group and individual policies simultaneously. Specifically, CoS comprises two main components: (a) the vector quantized group consensus module, which extracts discrete latent embeddings that represent the stable and discriminative group consensus, and (b) the group consensus-oriented strategy, which integrates the group policy using a hypernet and the individual policies using the group consensus, thereby promoting coordination at both the group and individual levels. Through empirical experiments on cooperative navigation tasks with both discrete and continuous spaces, as well as Google research football, we demonstrate that CoS outperforms state-of-the-art MARL algorithms and achieves better collaboration, thus providing a promising solution for achieving effective coordination in multi-agent systems.

==> 7-ethics.tex <==

 
% \setcounter{tocdepth}{2}
% \centering \LARGE
 \section*{\centering \LARGE Ethical Statement}

Our submission involves the development and evaluation of a cooperative multi-agent reinforcement learning method, which has potential implications in various applications, such as multi-player games, traffic signal control, and sensor networks. We have taken steps to ensure that our research does not infringe upon personal data privacy or contribute to any unethical practices such as those related to policing or military applications.

We use publicly available datasets for our experiments and have taken appropriate measures to ensure that any personal data has been anonymized or otherwise rendered non-identifiable. Additionally, we have implemented measures to ensure that our model does not infer personal information or engage in any discriminatory practices. Furthermore, we do not promote the use of our work for any unethical purposes, such as for surveillance or military purposes.

In summary, we recognize the importance of ethical considerations in machine learning and data mining and have taken steps to ensure that our work adheres to ethical principles and does not contribute to any negative societal impacts. We remain committed to ethical research practices and encourage others to do the same.
